X-ray cavities in a sample of 83 SPT-selected clusters of galaxies: Tracing the evolution of AGN feedback in clusters of galaxies out to z=1.2

X-ray cavities are key tracers of mechanical (or radio mode) heating arising from the active galactic nuclei (AGN) in brightest cluster galaxies. We report on a survey for X-ray cavities in 83 massive, high-redshift (0.4<z<1.2) clusters of galaxies selected by their Sunyaev-Zel'dovich signature in the South Pole Telescope data. Based on Chandra X-ray images, we find a total of 6 clusters having symmetric pairs of surface brightness depressions consistent with the picture of radio jets inflating X-ray cavities in the intracluster medium. The majority of these detections are of relatively low significance and require deeper follow-up data in order to be confirmed. Further, due to the limitations of Chandra at high redshift, this search misses small (<10 kpc), unresolved X-ray cavities at high (z>0.5) redshift. Despite these limitations, our results suggest that the power generated by AGN feedback in brightest cluster galaxies has remained unchanged for over half of the age of the Universe (>7 Gyrs at z=0.8). On average, the detected X-ray cavities have powers of 0.8-5*10^45 erg/s, enthalpies of 3-6*10^59 erg, and radii of 17 kpc. Integrating over 7 Gyrs, we find that the supermassive black holes in the brightest cluster galaxies may have accreted 10^8 to several 10^9M_sun of material to power these outflows. This level of accretion indicates that significant supermassive black hole growth may occur not only at early times, in the quasar era, but at late times as well. We also find that X-ray cavities at high-redshift may inject an excess heat of 0.1-1.0 keV per particle into the hot intracluster medium above and beyond the energy needed to offset cooling. This value is similar to the energy needed to preheat clusters, break self-similarity, and explain the excess entropy in hot atmospheres.

==> spt_authors.tex <==

\altaffiltext{\emailjhl}{juliehl@astro.umontreal.ca}
\altaffiltext{\UMon}{D\'{e}partement de Physique, Universit\'{e} de Montr\'{e}al, C.P. 6128, Succ. Centre-Ville, Montreal, Quebec H3C 3J7, Canada}
\altaffiltext{\KIPAC}{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, 452 Lomita Mall, Stanford, CA 94305}
\altaffiltext{\Stanford}{Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305}
\altaffiltext{\MIT}{Kavli Institute for Astrophysics and Space
Research, Massachusetts Institute of Technology, 77 Massachusetts Avenue,
Cambridge, MA 02139}
\altaffiltext{\KICPChicago}{Kavli Institute for Cosmological Physics, University of Chicago, 5640 South Ellis Avenue, Chicago, IL 60637}
\altaffiltext{\FNAL}{Fermi National Accelerator Laboratory, Batavia, IL 60510-0500}
\altaffiltext{\AAUChicago}{Department of Astronomy and Astrophysics, University of Chicago, 5640 South Ellis Avenue, Chicago, IL 60637}
\altaffiltext{\CfA}{Harvard-Smithsonian Center for Astrophysics,
60 Garden Street, Cambridge, MA 02138}
\altaffiltext{\SLAC}{SLAC National Accelerator Laboratory, 2575 Sand Hill Road, Menlo Park, CA 94025}
\altaffiltext{\ANL}{Argonne National Laboratory, High-Energy Physics Division, 9700 S. Cass Avenue, Argonne, IL, USA 60439}
\altaffiltext{\PhysicsUChicago}{Department of Physics, University of Chicago, 56 Ellis Avenue, Chicago, IL 60637}
%\altaffiltext{\UChicago}{University of Chicago,5640 South Ellis Avenue, Chicago, IL 60637}
%\altaffiltext{\McGill}{Department of Physics, McGill University, 3600 Rue University, Montreal, Quebec H3A 2T8, Canada}
%\altaffiltext{\Harvard}{Department of Physics, Harvard University, 17 Oxford Street, Cambridge, MA 02138}
\altaffiltext{\Munich}{Department of Physics,
Ludwig-Maximilians-Universit\"{a}t,
Scheinerstr.\ 1, 81679 M\"{u}nchen, Germany}
\altaffiltext{\ExcellenceCluster}{Excellence Cluster Universe,
Boltzmannstr.\ 2, 85748 Garching, Germany}
\altaffiltext{\Miss}{Department of Physics and Astronomy, University of Missouri, 5110 Rockhill Road, Kansas City, MO 64110}
%\altaffiltext{\EFIChicago}{Enrico Fermi Institute, University of Chicago, 5640 South Ellis Avenue, Chicago, IL 60637}
%\altaffiltext{\NIST}{NIST Quantum Devices Group, 325 Broadway Mailcode 817.03, Boulder, CO, USA 80305}
%\altaffiltext{\PUC}{Departamento de Astronomia y Astrosifica, Pontificia Universidad Catolica,Chile}
%\altaffiltext{\Caltech}{California Institute of Technology, 1200 E. California Blvd., Pasadena, CA 91125}
%\altaffiltext{\CIFAR}{Canadian Institute for Advanced Research, CIFAR Program in Cosmology and Gravity, Toronto, ON, M5G 1Z8, Canada}
%\altaffiltext{\illast}{Astronomy Department,University of Illinois at Urbana-Champaign,1002 W.\ Green Street,Urbana, IL 61801 USA}
%\altaffiltext{\illphy}{Department of Physics,University of Illinois Urbana-Champaign,1110 W.\ Green Street,Urbana, IL 61801 USA}
\altaffiltext{\Berkeley}{Department of Physics,University of California, Berkeley, CA 94720}
\altaffiltext{\Melbourne}{School of Physics, University of Melbourne, Parkville, VIC 3010, Australia}
%\altaffiltext{\MPE}{Max-Planck-Institut f\"{u}r extraterrestrische Physik,Giessenbachstr.\ 85748 Garching, Germany}
%\altaffiltext{\UFlorida}{Department of Astronomy, University of Florida, Gainesville, FL 32611}
%\altaffiltext{\Colorado}{Department of Astrophysical and Planetary Sciences and Department of Physics,University of Colorado,Boulder, CO 80309}
%\altaffiltext{\LeidenObservatory}{Leiden Observatory, Leiden University, Niels Bohrweg 2, 2333 CA, Leiden, the Netherlands}
%\altaffiltext{\Davis}{Department of Physics, University of California, One Shields Avenue, Davis, CA 95616}
%\altaffiltext{\LBNL}{Physics Division,Lawrence Berkeley National Laboratory,Berkeley, CA 94720}
%\altaffiltext{\Arizona}{Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721}
\altaffiltext{\CaseWestern}{Physics Department, Center for Education and Research in Cosmology and Astrophysics, Case Western Reserve University, Cleveland, OH 44106}
\altaffiltext{\AIfA}{Argelander-Institut f{\"u}r Astronomie, Auf dem H{\"u}gel 71, D-53121 Bonn, Germany}
\altaffiltext{\Michigan}{Department of Physics, University of Michigan, 450 Church Street, Ann  Arbor, MI, 48109}
%\altaffiltext{\Minnesota}{Physics Department, University of Minnesota, 116 Church Street S.E., Minneapolis, MN 55455}

%\altaffiltext{\STScI}{Space Telescope Science Institute, 3700 San Martin, Dr., Baltimore, MD 21218}
%\altaffiltext{\SAIC}{Liberal Arts Department, School of the Art Institute of Chicago, 112 S Michigan Ave, Chicago, IL 60603}
%\altaffiltext{\LLNL}{Institute of Geophysics and Planetary Physics, Lawrence Livermore National Laboratory, Livermore, CA 94551}
%\altaffiltext{\Dunlap}{Dunlap Institute for Astronomy \& Astrophysics, University of Toronto, 50 St George St, Toronto, ON, M5S 3H4, Canada}
%\altaffiltext{\Toronto}{Department of Astronomy \& Astrophysics, University of Toronto, 50 St George St, Toronto, ON, M5S 3H4, Canada}
%\altaffiltext{\BCCP}{Berkeley Center for Cosmological Physics,Department of Physics, University of California, and Lawrence Berkeley National Labs, Berkeley, CA 94720}
\altaffiltext{\Korea}{Korea Astronomy \& Space Science Institute, Daejeon, Republic of Korea}
\altaffiltext{\Hawaii}{Institute for Astronomy, University of Hawaii at Manoa, Honolulu, HI 96822, USA}

\altaffiltext{\CTIO}{Cerro Tololo Inter-American Observatory, Casilla 603, La Serena, Chile}


\def\emailjhl{$\dagger$}
\def\UMon{1}
\def\KIPAC{2}
\def\Stanford{3}
\def\MIT{4}
\def\KICPChicago{5}
\def\FNAL{6}
\def\AAUChicago{7}
\def\CfA{8}
\def\SLAC{9}
\def\ANL{10}
\def\PhysicsUChicago{11}
%\def\UChicago{12}
\def\AIfA{18}
%\def\McGill{14}
%\def\Harvard{15}
\def\Munich{12}
\def\ExcellenceCluster{13}
\def\Miss{14}
%\def\EFIChicago{19}
%\def\NIST{20}
%\def\PUC{21}
%\def\Caltech{22}
%\def\CIFAR{23}
%\def\illast{24}
%\def\illphy{25}
\def\Berkeley{15}
%\def\MPE{27}
%\def\UFlorida{28}
%\def\Colorado{29}
%\def\LeidenObservatory{30}
%\def\Davis{31}
%\def\LBNL{32}
%\def\Arizona{33}
\def\Michigan{19}
%\def\Minnesota{35}
\def\Melbourne{16}
%\def\STScI{37}
\def\CaseWestern{17}
%\def\SAIC{39}
%\def\LLNL{40}
%\def\Dunlap{41}
%\def\Toronto{42}
%\def\BCCP{43}
\def\CTIO{22}
\def\Korea{20}
\def\Hawaii{21}


\author{
J.~Hlavacek-Larrondo\altaffilmark{\UMon,\KIPAC,\Stanford,\emailjhl},
M.~McDonald\altaffilmark{\MIT},
B.~A.~Benson\altaffilmark{\KICPChicago,\FNAL,\AAUChicago},
W.~R.~Forman\altaffilmark{\CfA},
S.~W.~Allen\altaffilmark{\KIPAC,\Stanford,\SLAC},
L.~E.~Bleem\altaffilmark{\KICPChicago,\ANL,\PhysicsUChicago},
%K.~A.~Aird\altaffilmark{\UChicago},
%%D.~E.~Applegate\altaffilmark{\AIfA},
M.~L.~N.~Ashby\altaffilmark{\CfA},
%M.~Bautz\altaffilmark{\MIT},
%%M.~Bayliss\altaffilmark{\CfA,\Harvard},
S.~Bocquet\altaffilmark{\Munich,\ExcellenceCluster},
M.~Brodwin\altaffilmark{\Miss},
%%J.~E.~Carlstrom\altaffilmark{\ANL,\KICPChicago,\PhysicsUChicago,\AAUChicago,\EFIChicago}, 
%C.~L.~Chang\altaffilmark{\ANL,\KICPChicago,\EFIChicago}, 
%I.~Chiu\altaffilmark{\Munich,\ExcellenceCluster},
%H.~M.~Cho\altaffilmark{\NIST}, 
%A.~Clocchiatti\altaffilmark{\PUC},
%A.~T.~Crites\altaffilmark{\KICPChicago,\AAUChicago,\Caltech},
%S.~Desai\altaffilmark{\Munich,\ExcellenceCluster},
J.~P.~Dietrich\altaffilmark{\Munich,\ExcellenceCluster},
%M.~A.~Dobbs\altaffilmark{\McGill,\CIFAR},
%R.~J.~Foley\altaffilmark{\CfA,\illast,\illphy},
%E.~M.~George\altaffilmark{\Berkeley,\MPE},
%M.~D.~Gladders\altaffilmark{\KICPChicago,\AAUChicago},
%A.~H.~Gonzalez\altaffilmark{\UFlorida},
%N.~W.~Halverson\altaffilmark{\Colorado},
%T.~de~Haan\altaffilmark{\McGill},
%C.~Hennig\altaffilmark{\Munich,\ExcellenceCluster},
%H.~Hoekstra\altaffilmark{\LeidenObservatory}, 
%G.~P.~Holder\altaffilmark{\McGill},
%W.~L.~Holzapfel\altaffilmark{\Berkeley},
%J.~D.~Hrubes\altaffilmark{\UChicago},
C.~Jones\altaffilmark{\CfA},
%R.~Keisler\altaffilmark{\KICPChicago,\PhysicsUChicago,\KIPAC,\Stanford},
%L.~Knox\altaffilmark{\Davis},
%A.~T.~Lee\altaffilmark{\Berkeley,\LBNL},
%E.~M.~Leitch\altaffilmark{\KICPChicago,\AAUChicago},
J.~Liu\altaffilmark{\Munich,\ExcellenceCluster},
%M.~Lueker\altaffilmark{\Caltech,\Berkeley},
%D.~Luong-Van\altaffilmark{\UChicago},
%%A.~Mantz\altaffilmark{\KICPChicago},
%D.~P.~Marrone\altaffilmark{\Arizona},
%J.~J.~McMahon\altaffilmark{\Michigan},
%S.~S.~Meyer\altaffilmark{\KICPChicago,\PhysicsUChicago,\AAUChicago,\EFIChicago},
%L.~Mocanu\altaffilmark{\KICPChicago,\AAUChicago},
%J.~J.~Mohr\altaffilmark{\Munich,\ExcellenceCluster,\MPE},
%S.~S.~Murray\altaffilmark{\CfA},
%S.~Padin\altaffilmark{\KICPChicago,\AAUChicago,\Caltech},
%C.~Pryke\altaffilmark{\Minnesota}, 
C.~L.~Reichardt\altaffilmark{\Berkeley,\Melbourne},
%A.~Rest\altaffilmark{\STScI},
%J.~Ruel\altaffilmark{\Harvard},
%J.~E.~Ruhl\altaffilmark{\CaseWestern}, 
B.~R.~Saliwanchik\altaffilmark{\CaseWestern}, 
A.~Saro\altaffilmark{\Munich},
%J.~T.~Sayre\altaffilmark{\CaseWestern}, 
%K.~K.~Schaffer\altaffilmark{\KICPChicago,\EFIChicago,\SAIC}, 
T.~Schrabback\altaffilmark{\AIfA},
%E.~Shirokoff\altaffilmark{\Caltech,\Berkeley}, 
J.~Song\altaffilmark{\Michigan,\Korea},
%H.~G.~Spieler\altaffilmark{\LBNL},
B.~Stalder\altaffilmark{\CfA,\Hawaii},
%S.~A.~Stanford\altaffilmark{\Davis,\LLNL},
%Z.~Staniszewski\altaffilmark{\Caltech,\CaseWestern},
%A.~A.~Stark\altaffilmark{\CfA}, 
%K.~T.~Story\altaffilmark{\KICPChicago,\PhysicsUChicago},
%K.~Vanderlinde\altaffilmark{\Dunlap,\Toronto},
%J.~D.~Vieira\altaffilmark{\illast,\illphy},
A. Vikhlinin\altaffilmark{\CfA},
%R.~Williamson\altaffilmark{\KICPChicago,\AAUChicago,\Caltech}, 
%O.~Zahn\altaffilmark{\Berkeley,\BCCP},
and
A.~Zenteno\altaffilmark{\Munich,\CTIO}
}

